Not All Countries Celebrate Thanksgiving: On the Cultural Dominance in Large Language Models

This paper identifies a cultural dominance issue within large language models (LLMs) due to the predominant use of English data in model training (e.g., ChatGPT). LLMs often provide inappropriate English-culture-related answers that are not relevant to the expected culture when users ask in non-English languages. To systematically evaluate the cultural dominance issue, we build a benchmark of concrete (e.g., holidays and songs) and abstract (e.g., values and opinions) cultural objects. Empirical results show that the representative GPT models suffer from the culture dominance problem, where GPT-4 is the most affected while text-davinci-003 suffers the least from this problem. Our study emphasizes the need to critically examine cultural dominance and ethical consideration in their development and deployment. We show that two straightforward methods in model development (i.e., pretraining on more diverse data) and deployment (e.g., culture-aware prompting) can significantly mitigate the cultural dominance issue in LLMs.

==> Sections/4_Discussions.tex <==
\section{Discussion}

\subsection{Culture Invasion and Exchange}

Alerting culture invasion does not mean refusing culture exchange. With the process of globalization, the exchanges between various countries are getting closer and closer, and cultural exchanges are inevitable. Different from cultural invasion, cultural exchange is generally seen as a positive and constructive process whereby different cultures share, adapt, and integrate elements from each other. The interaction often leads to mutual understanding, tolerance, and appreciation of other cultures. Cultural invasion, on the other hand, refers to the domination of one culture over another. This can lead to the weakening or even disappearance of subordinated cultures and is often viewed negatively, as it may lead to the loss of cultural diversity and heritage, and impose a form of cultural homogeneity.

While cultural exchange is inevitable and generally positive, it's crucial to ensure it doesn't turn into a cultural invasion. There should be respect for cultural diversity and active measures to preserve and promote indigenous and local cultures. Ensuring that no culture is marginalized or dominated by another is key to maintaining the rich tapestry of global cultural diversity. The goal should not be to prevent cultural exchange, but to ensure it happens on a fair and respectful basis, without leading to the extinction or marginalization of any culture.

\subsection{Language and Culture}

We need to mention that a single language can encompass multiple cultures. As languages spread across regions, they adapt and evolve, adopting new vocabularies, accents, idioms, and linguistic rules from the cultures they interact with. For example, English, widely spoken worldwide, includes a plethora of cultural nuances, encapsulated within its myriad dialects and sociolects. American English, British English, Australian English, and Indian English, to name a few, each reflects the distinct cultures they belong to. Even within the same region, different groups of people can have different cultures.

However, we posit that the cultural disparities among groups speaking the same language are often less than those among groups speaking different languages. This is attributed to the role of language as a pivotal medium and delineator in the transmission and fusion of cultures. The purpose of this paper is not to argue that groups speaking the same language invariably share identical cultural features, but to highlight an alternative issue: when non-English users communicate with ChatGPT in their native language, the primary cultural output from ChatGPT remains entrenched in English culture. Such cultural invasion presents potential issues that warrant attention from both the academic and industrial.


